Meta-Learning of NAS for Few-shot Learning in Medical Image Applications

Deep learning methods have been successful in solving tasks in machine learning and have made breakthroughs in many sectors owing to their ability to automatically extract features from unstructured data. However, their performance relies on manual trial-and-error processes for selecting an appropriate network architecture, hyperparameters for training, and pre-/post-procedures. Even though it has been shown that network architecture plays a critical role in learning feature representation feature from data and the final performance, searching for the best network architecture is computationally intensive and heavily relies on researchers' experience. Automated machine learning (AutoML) and its advanced techniques i.e. Neural Architecture Search (NAS) have been promoted to address those limitations. Not only in general computer vision tasks, but NAS has also motivated various applications in multiple areas including medical imaging. In medical imaging, NAS has significant progress in improving the accuracy of image classification, segmentation, reconstruction, and more. However, NAS requires the availability of large annotated data, considerable computation resources, and pre-defined tasks. To address such limitations, meta-learning has been adopted in the scenarios of few-shot learning and multiple tasks. In this book chapter, we first present a brief review of NAS by discussing well-known approaches in search space, search strategy, and evaluation strategy. We then introduce various NAS approaches in medical imaging with different applications such as classification, segmentation, detection, reconstruction, etc. Meta-learning in NAS for few-shot learning and multiple tasks is then explained. Finally, we describe several open problems in NAS.

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}

  \section*{Sir Stanley Davidson (1894--1981)}

  One or more blank lines denote the end of a paragraph.  The ends of\index{index}
  words and sentences are marked by spaces. It doesn't matter how many
  spaces you type; one is as good as 100.  The end of a line counts as
  a space.

\end{biography}


==> chapter2.tex <==
\cleardoublepage

\begin{frontmatter}
\chapter{Capsule Networks for Medical Imaging}\label{chap2}
\subchapter{Chapter Subtitle}

\begin{aug}
\author[addressrefs={ad1,ad2}]%
  {\fnm{Firstname}   \snm{Surname}}%
  %{\fnm{Firstname}   \snm{Surname}\footnote{This is author footnote}}%
\author[addressrefs={ad2}]%
 {\fnm{Firstname} \snm{Surname}}%
\address[id=ad1]%
  {Short Address}%
\address[id=ad2]%
  {Long Address}%
\end{aug}


% \minitoc

%
\begin{chapterpoints}%[Chapter Points]
\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space. \cite{cheng2020hierarchical}

\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
\end{chapterpoints}

\begin{dispquote}

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
  
  \source{Name}

\end{dispquote}

\end{frontmatter}


\section{Capsule Network: Basic}\label{sec2.1}
\section{2D Capsule Network}
\section{3D Capsule Network}
\section{Comparison between CapsNets and CNNs}


==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}
  \name{Greg N. Gregoriou} is Professor of Finance in the School of
  Business and Economics at State University of New York at
  Plattsburgh. He obtained his Ph.D. (finance) from the University of
  Quebec at Montreal and is hedge-fund editor for the peer-reviewed
  scientific journal Derivatives Use, Trading and Regulation and
  editorial board member for the Journal of Wealth Management, and the
  Journal of Risk and Financial Institutions. He has written more than
  50 articles on hedge funds and managed futures in various U.S. and
  U.K. peer-reviewed publications, including (among others) the
  Journal of Portfolio Management, Journal of Derivatives Accounting,
  Journal of Futures Markets, European Journal of Operational
  Research, Annals of Operations Research, European Journal of
  Finance, and Journal of Asset Management. He has edited 18 books for
  Elsevier, Wiley, Palgrave-MacMillan, and Risk and has coauthored one
  book for Wiley.

  \name{Donald F. Dansereau} Department of Psychology, Texas Christian
  University, Fort worth, Texas

  \name{Ruth Garner} Department of Educational Psychology, Texas A \&
  M University, College Station, Texas
\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}

% Text ...

